A structured approach to VO reconfigurations through Policies

One of the strength of Virtual Organisations is their ability to dynamically and rapidly adapt in response to changing environmental conditions. Dynamic adaptability has been studied in other system areas as well and system management through policies has crystallized itself as a very prominent solution in system and network administration. However, these areas are often concerned with very low-level technical aspects. Previous work on the APPEL policy language has been aimed at dynamically adapting system behaviour to satisfy end-user demands and - as part of STPOWLA - APPEL was used to adapt workflow instances at runtime. In this paper we explore how the ideas of APPEL and STPOWLA can be extended from workflows to the wider scope of Virtual Organisations. We will use a Travel Booking VO as example.

==> eptcsdata.tex <==
\providecommand{\firstpage}{22}
\providecommand{\publicationstatus}{Jeremy Bryans and John Fitzgerald (Eds.): \\
Formal Aspects of Virtual Organisations 2011 (FAVO 2011)\\
EPTCS 83, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.83.3}{10.4204/EPTCS.83.3}}
\pdfoutput=1

